Distributed Hypothesis Testing and Social Learning in Finite Time with a Finite Amount of Communication

We consider the problem of distributed hypothesis testing (or social learning) where a network of agents seeks to identify the true state of the world from a finite set of hypotheses, based on a series of stochastic signals that each agent receives. Prior work on this problem has provided distributed algorithms that guarantee asymptotic learning of the true state, with corresponding efforts to improve the rate of learning. In this paper, we first argue that one can readily modify existing asymptotic learning algorithms to enable learning in finite time, effectively yielding arbitrarily large (asymptotic) rates. We then provide a simple algorithm for finite-time learning which only requires the agents to exchange a binary vector (of length equal to the number of possible hypotheses) with their neighbors at each time-step. Finally, we show that if the agents know the diameter of the network, our algorithm can be further modified to allow all agents to learn the true state and stop transmitting to their neighbors after a finite number of time-steps.

==> old.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Model and Problem Formulation}
\label{sec:model}
\textbf{Network Model:} We consider a setting comprising of a group of agents $\mathcal{V}=\{1,2,\ldots,n\}$. At certain specific time-steps (to be decided by a time-triggered communication schedule), these agents
interact with each other over a directed graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$. An edge $(i,j)\in\mathcal{E}$ indicates that agent $i$ can directly transmit information to agent $j$; in such a case, agent $i$ will be called a neighbor of agent $j$. The set of all neighbors of agent $i$ will be denoted $\mathcal{N}_i$. For a strongly-connected graph $\mathcal{G}$, we will use $d(i,j)$ to denote the length of the shortest directed path from agent $i$ to agent $j$, and $\bar{d}({\mathcal{G}})$ to denote the diameter of the graph.\footnote{A graph is said to be strongly-connected if it has a directed path between every pair of agents; the diameter of such a graph is the length of the longest shortest path between the agents.}

\textbf{Observation Model:} Let $\Theta=\{\theta_1,\theta_2,\ldots,\theta_m\}$ denote $m$ possible states of the world, with each state representing a hypothesis. A specific state $\theta^{\star}\in\Theta$, referred to as the true state of the world, gets realized. Conditional on its realization, at each time-step $t\in\mathbb{N}_{+}$, every agent $i\in\mathcal{V}$  privately observes a signal $s_{i,t}\in\mathcal{S}_i$, where $\mathcal{S}_i$ denotes the signal space of agent $i$.\footnote{We use $\mathbb{N}$ and $\mathbb{N}_{+}$ to refer to the set of non-negative integers and positive integers, respectively.} The joint observation profile so generated across the network is denoted ${s}_{t}=(s_{1,t},s_{2,t},\ldots,s_{n,t})$, where $s_t\in\mathcal{S}$, and $\mathcal{S}=\mathcal{S}_1\times\mathcal{S}_2\times\ldots \mathcal{S}_n$. 
Specifically, the signal $s_{t}$ is generated based on a conditional likelihood function $l(\cdot|\theta^{\star})$, the $i$-th marginal of which is denoted $l_i(\cdot|\theta^{\star})$, and is available to agent $i$. The signal structure of each agent $i\in\mathcal{V}$ is thus characterized by a family of parameterized marginals $l_i=\{l_i(w_i|\theta): \theta\in\Theta, w_i\in\mathcal{S}_i\}$. We make certain standard assumptions \cite{jad1,jad2,shahin,nedic,lalitha}: (i) The signal space of each agent $i$, namely $\mathcal{S}_i$, is finite. (ii) Each agent $i$ has knowledge of its local likelihood functions $\{l_i(\cdot|\theta_p)\}_{p=1}^{m}$, and it holds that $l_i(w_i|\theta) > 0, \forall w_i\in\mathcal{S}_i$, and $\forall \theta \in \Theta$. (iii) The observation sequence of each agent is described by an i.i.d. random process over time; however, at any given time-step, the observations of different agents may potentially be correlated. (iv) There exists a fixed true state of the world $\theta^{\star}\in\Theta$ (that is unknown to the agents) that generates the observations of all the agents. The probability space for our model is denoted $(\Omega,\mathcal{F},\mathbb{P}^{\theta^{\star}})$, where $\Omega\triangleq\{\omega: \omega=(s_1,s_2,\ldots), \forall s_t\in\mathcal{S}, \forall t \in \mathbb{N}_{+}\}$, $\mathcal{F}$ is the $\sigma$-algebra generated by the observation profiles, and $\mathbb{P}^{\theta^{\star}}$ is the probability measure induced by sample paths in $\Omega$. Specifically, $\mathbb{P}^{\theta^{\star}}=\prod \limits_{t=1}^{\infty}l(\cdot|\theta^{\star})$. We will use the abbreviation a.s. to indicate almost sure occurrence of an event w.r.t. $\mathbb{P}^{\theta^{\star}}$.

Given the above setting, the goal of each agent in the network is to eventually learn the true state of the world $\theta^{\star}$. However, the signal structure of any given agent is in general only partially informative, thereby precluding this task from being achieved by any agent in isolation. Specifically, let $\Theta^{\theta^{\star}}_i\triangleq\{\theta\in\Theta : l_i(w_i|\theta)=l_i(w_i|\theta^{\star}), \forall w_i\in\mathcal{S}_i\}$  represent the set of hypotheses that are \textit{observationally equivalent} to the true state $\theta^{\star}$ from the perspective of agent $i$. An agent $i$ is deemed partially informative about the truth if  $|\Theta^{\theta^{\star}}_i| > 1$. Since potentially every agent can be partially informative in the sense described above, inter-agent communications become necessary for each agent to learn the truth. 

In this context, our \textbf{objectives} in this paper are to develop an understanding of (i) the amount of leeway that the above problem affords in terms of sparsifying inter-agent communications without compromising the objective of learning the truth, and (ii) the trade-offs between sparse communication and the rate of learning. To this end, we recall the following definition from \cite{mitraACC19} that will prove useful in our subsequent developments. 



Throughout the rest of the paper, we will use $K_i(\theta_p,\theta_q)$
as a shorthand for $D(l_i(\cdot|\theta_p)||l_i(\cdot|\theta_q))$.



\section{A Communication-Efficient Learning Rule}
\label{sec:Algo}
In this section, we formally introduce a simple time-triggered belief update rule parameterized by a constant $a\in\mathbb{N}_{+}$ that determines the frequency of communication (to be made more precise below). In order to collaboratively learn the true state of the world, every agent $i$ maintains a local belief vector $\boldsymbol{\pi}_{i,t}$, and an actual belief vector $\boldsymbol{\mu}_{i,t}$, each of which are probability distributions over the hypothesis set $\Theta$. These vectors are initialized with $\pi_{i,0}(\theta)>0,\mu_{i,0}(\theta)>0, \forall \theta\in\Theta,\forall i\in\mathcal{V}$ (but otherwise arbitrarily), and subsequently updated as follows. 
\begin{itemize}
\item \underline{\textbf{Update of the local beliefs}:} At each time-step $t+1\in\mathbb{N}_{+}$, the local belief vectors are updated based on a standard Bayesian rule:
\begin{equation}
\pi_{i,t+1}(\theta)=\frac{l_i(s_{i,t+1}|\theta)\pi_{i,t}(\theta)}{\sum  \limits_{p=1}^{m} l_i(s_{i,t+1}|\theta_p)\pi_{i,t}(\theta_p)}.
\label{eqn:Bayes}
\end{equation}
\item \underline{\textbf{Update of the actual beliefs}:}
Let $\mathbb{I}={\{t_k\}}_{ k\in\mathbb{N}_{+}}$ denote a sequence of time-steps satisfying $t_{k+1}-t_k=a^k, \forall k\in\mathbb{N}_{+}$, with $t_1=1$. If $t+1\in\mathbb{I}$, then $\boldsymbol{\mu}_{i,t+1}$ is updated as
\begin{equation}
\mu_{i,t+1}(\theta)=\frac{\min\{\{\mu_{j,t}(\theta)\}_{{j\in\mathcal{N}_i}},\pi_{i,t+1}(\theta)\}}{\sum\limits_{p=1}^{m}\min\{\{\mu_{j,t}(\theta_p)\}_{{j\in\mathcal{N}_i}},\pi_{i,t+1}(\theta_p)\}}.
\label{eqn:update1}
\end{equation}
If $t+1\notin\mathbb{I}$,  $\boldsymbol{\mu}_{i,t+1}$ is simply held constant as follows:
\begin{equation}
    \mu_{i,t+1}(\theta)=\mu_{i,t}(\theta).
    \label{eqn:update2}
\end{equation}
\end{itemize}
In words, while the local beliefs are updated at every time-step, the actual beliefs are updated only at time-steps that belong to the set $\mathbb{I}$, i.e., an agent $i\in\mathcal{V}$ is allowed to transmit  $\boldsymbol{\mu}_{i,t}$ to its out-neighbors, and receive $\boldsymbol{\mu}_{j,t}$ from each in-neighbor $j$ in $\mathcal{G}$ if and only if $t+1\in\mathbb{I}$. When $a=1$, the actual beliefs get updated as per \eqref{eqn:update1} at \textit{every} time-step, and we recover the rule proposed in  \cite{mitraACC19}. When $a>1$, note that the inter-communication intervals grow exponentially at a rate dictated by the parameter $a$. Our goal in this paper is to precisely characterize the impact of such sparse communication on the asymptotic rate of learning of each agent. Prior to doing so, a few comments are in order.

First, notice that the data-aggregation rule in \eqref{eqn:update1} is based on a min-protocol, as opposed to any form of ``belief-averaging" commonly employed in the existing distributed learning literature \cite{jad1,jad2,shahin,nedic,lalitha}. Essentially, while the local belief updates \eqref{eqn:Bayes} capture what an agent can learn by itself, the actual belief updates \eqref{eqn:update1} incorporate information from the rest of the network. As demonstrated by Corollary \ref{thm:corollary} in the next section, when $a=1$, such a min-protocol yields better asymptotic learning rates than all existing schemes. This motivates us to use a belief update rule of the form \eqref{eqn:update1} for studying the case when $a>1$. 
\iffalse
Second, a natural question arises as to why the actual beliefs are not updated in the intervals between successive communications based on \eqref{eqn:update1}, using $\mu_{i,t}(\theta)$ and $\pi_{i,t+1}(\theta)$ to perform the recursion. To see why this is not done, consider a binary hypothesis testing example where $\Theta=\{\theta_1,\theta_2\}$, and $\theta_1$ is the true state of the world. Consider an agent $i\in\mathcal{V}\setminus\mathcal{S}(\theta_1,\theta_2)$. Since this agent has no discriminatory power, it can be easily shown that the local belief vector (evolving as per \eqref{eqn:Bayes}) for this agent satisfies $\boldsymbol{\pi_{i,t}}=\boldsymbol{\pi_{i,0}}, \forall t\in \mathbb{N}_{+}$. Now suppose agent $i$ updates $\boldsymbol{\mu_{i,t}}$ during the inter-communication intervals based on the following rule (instead of \eqref{eqn:update2}):
\begin{equation}
\mu_{i,t+1}(\theta)=\frac{\min\{\mu_{i,t}(\theta),\pi_{i,t+1}(\theta)\}}{\sum\limits_{p=1}^{2}\min\{\mu_{i,t}(\theta_p),\pi_{i,t+1}(\theta_p)\}}.
\label{eqn:counter}
\end{equation}
The above rule has the effect of aligning the actual belief vector $\boldsymbol{\mu_{i,t}}$ towards the local belief vector $\boldsymbol{\pi_{i,t}}=\boldsymbol{\pi_{i,0}}$, i.e., $\mu_{i,t}(\theta_2)$  will gradually approach $\pi_{i,0}(\theta_2)$ over the interval between communications. Since such intervals grow exponentially, such a phenomenon will eventually occur. Consequently, if an uninformative agent initially has a high local belief on the false state $\theta_2$, its actual belief will get pulled towards this value during the period when it gets no additional information from its neighbors. This is clearly undesirable. It is precisely this consideration that motivates us to employ rule \eqref{eqn:update1} \textit{only} when an agent $i$ can evaluate the quality of its local beliefs in the light of information from neighbors.
\fi
Second, we note that the proposed time-triggered protocol is simple, easy to implement and computationally cheap. At the same time, the exponentially growing intervals afford a much sparser communication schedule relative to related literature. Third, while one can potentially consider extensions of this algorithm that account for asynchronicity, communication failures, delays etc., we focus on the scheme here in order to (i) concretely isolate the trade-off between sparse communication and the quality of learning as measured by the asymptotic learning rates, and (ii) provide insights into how the network structure impacts such rates. A final comment needs to made regarding the choice of achieving communication-efficiency by cutting down on communication rounds as opposed to truncating the number of bits exchanged per communication round, an approach pursued in quantization-based schemes \cite{suresh}. As argued in \cite{opt2}, communication latency acts as the bottleneck of overall performance and dominates message-size dependent transmission latency when it comes to transmitting small messages, such as the $m$-dimensional actual belief vectors in our setting. This justifies our sparse communication scheme.
With these points in mind, we proceed to the analysis of the algorithm developed in this section. 





 \textbf{Implications of Corollary \ref{thm:corollary}}: In sharp contrast to the case when $a>1$, Corollary \ref{thm:corollary} indicates that when communication occurs at every time-step (i.e., $a=1$), the asymptotic learning rates are \textit{network-structure independent}, and \textit{identical} for each agent. Since this case represents the standard distributed hypothesis testing setup studied in literature, it becomes important to know how such rates compare with those resulting from existing  ``belief-averaging" schemes \cite{jad1,jad2,shahin,lalitha,nedic}. To this end, we note that under the same set of assumptions as in Theorem \ref{thm:main}, both linear \cite{jad1,jad2} and log-linear \cite{shahin,lalitha,nedic} opinion pooling lead to an asymptotic rate of rejection of the form $\sum_{i\in\mathcal{V}}\nu_iK_i(\theta^{\star},\theta)$ for each false hypothesis $\theta\in\Theta\setminus\{\theta^{\star}\}$, and the rate is identical for each agent. Here, $\nu_i$ represents the eigenvector centrality of agent $i\in\mathcal{V}$. It is well known that for a strongly-connected graph, $\nu_i>0, \forall i\in \mathcal{V}$. Thus, based on the above discussion, and referring to \eqref{eqn:asymprate2}, we conclude that a significant contribution of the algorithm proposed in this paper is that it yields \textit{strictly better} asymptotic learning rates than those existing in the literature, for the standard setting when $a=1$.\footnote{Recently, in \cite{mitraTAC19}, we showed that this result continues to hold even if the underlying graph changes with time, but satisfies a mild joint-strong connectivity condition.}



\section{Proof of the Main Result}
\label{sec:proofs}
In order to prove Theorem \ref{thm:main}, we require a few intermediate results. The first one is a standard consequence of Bayesian updating,  and characterizes the behavior of the local belief trajectories generated via \eqref{eqn:Bayes}; for a proof, see \cite{mitraACC19}. 

\begin{lemma}
 Suppose the conditions in Theorem \ref{thm:main} hold, and the learning rule given by \eqref{eqn:Bayes}, \eqref{eqn:update1}, and \eqref{eqn:update2} is employed by each agent. Then, there exists a set $\bar{\Omega}\subseteq\Omega$ with the following properties: (i) $\mathbb{P}^{\theta^{\star}}(\bar{\Omega})=1$, and (ii) for each $\omega\in\bar{\Omega}$, there exist constants $\eta(\omega)\in(0,1)$ and $t'(\omega)\in(0,\infty)$ such that
\begin{equation}
\pi_{i,t}(\theta^{\star}) \geq \eta(\omega), \mu_{i,t}(\theta^{\star}) \geq \eta(\omega), \forall t \geq t'(\omega),\forall i\in\mathcal{V}.
\label{eqn:lowerbound}
    \end{equation}
\label{lemma:bound}
\end{lemma}
\iffalse
\begin{proof} Let $\bar{\Omega}\subseteq\Omega$ denote the set of sample paths for which the assertions in Lemma \ref{lemma:Bayes} hold for each false hypothesis $\theta\in\Theta\setminus\{\theta^{\star}\}$. Based on Lemma \ref{lemma:Bayes}, we note that $\mathbb{P}^{\theta^{\star}}(\bar{\Omega})=1$. Consequently, to prove the result, it suffices to establish the existence of $\eta(\omega) \in (0,1)$, and $t'(\omega)\in (0,\infty)$ such that \eqref{eqn:lowerbound} holds for each sample path $\omega \in \bar{\Omega}$. To this end, pick an arbitrary sample path $\omega\in\bar{\Omega}.$ We first argue that the local beliefs of every agent on the true state $\theta^{\star}$ are bounded away from $0$ on $\omega$. To see this, pick any agent $i\in\mathcal{V}$. Suppose there exists some $\theta\in\Theta\setminus\{\theta^{\star}\}$ for which $i\in\mathcal{S}(\theta^{\star},\theta)$. Then, based on our choice of $\omega$, it follows directly from Lemma \ref{lemma:Bayes} that $\pi_{i,\infty}(\theta^{\star})\geq\pi_{i,0}(\theta^{\star})>0$, where the last inequality follows from condition (iii) in Theorem \ref{thm:main}. In particular, given the structure of the update rule \eqref{eqn:Bayes}, it follows that $\pi_{i,t}(\theta^{\star}) > 0$ for all time (since if $\pi_{i,t}(\theta^{\star})=0$ at any instant, then the corresponding belief would remain at $0$ for all subsequent time-steps, thereby violating the fact that $\pi_{i,\infty}(\theta^{\star})\geq\pi_{i,0}(\theta^{\star})>0$). If there exists no  $\theta\in\Theta\setminus\{\theta^{\star}\}$ for which $i\in\mathcal{S}(\theta^{\star},\theta)$, then every hypothesis in $\Theta$ is observationally equivalent to $\theta^{\star}$ from the point of view of agent $i$. In this case, it is easy to see that based on \eqref{eqn:Bayes}, $\boldsymbol{\pi}_{i,t}=\boldsymbol{\pi}_{i,0}, \forall t\in\mathbb{N}_{+}$. In particular, this implies $\pi_{i,t}(\theta^{\star})=\pi_{i,0}(\theta^{\star})>0, \forall t \in \mathbb{N}_{+}$. This establishes our claim that on $\omega$, the local beliefs of all the agents remain bounded away from $0$. 

 To proceed, define $\gamma_1\triangleq\min_{i\in\mathcal{V}} \pi_{i,0}(\theta^{\star})>0$, where the inequality follows from condition (iii) in Theorem \ref{thm:main}. Pick a small number $\delta > 0$ such that $\delta < \gamma_1$, and notice that our discussion concerning the evolution of the local beliefs readily implies the existence of a time-step $t'(\omega)$, such that for all $t \geq t'(\omega)$, $\pi_{i,t}(\theta^{\star}) \geq  \gamma_1-\delta > 0, \forall i\in\mathcal{V}$. Now define $\gamma_2(\omega)\triangleq\min_{i\in\mathcal{V}}\{\mu_{i,t'(\omega)}(\theta^{\star})\}$, and observe that $\gamma_2(\omega) > 0$. This observation follows from the fact that given the structure of the update rules \eqref{eqn:update1} and \eqref{eqn:update2}, and condition (iii) in Theorem \ref{thm:main},  $\gamma_2(\omega)$ can equal $0$
if and only if some agent in the network sets its local belief on $\theta^{\star}$ to $0$ at some time-step prior to $t'(\omega)$. However, this possibility is ruled out in view of the previously established fact that on $\omega$, $\pi_{i,t}(\theta^{\star})>0, \forall t\in\mathbb{N}, \forall i\in\mathcal{V}$.
Let $\eta(\omega)=\min\{\gamma_1-\delta,\gamma_2(\omega)\} > 0$. It is apparent from the preceding discussion that $\pi_{i,t}(\theta^{\star})\geq\eta(\omega),\forall t\geq t'(\omega),\forall i\in\mathcal{V}$. It remains to establish a similar result for the actual beliefs $\mu_{i,t}(\theta^{\star})$.
To this end, let $\bar{t}(\omega) > t'(\omega)$ be the first time-step following $t'(\omega)$ that belongs to the set $\mathbb{I}$. Based on \eqref{eqn:update2}, notice that $\mu_{i,t}(\theta^{\star}) \geq \eta(\omega)$ for all $t\in[t'(\omega),\bar{t}(\omega))$, and for each $i\in\mathcal{V}$. Based on \eqref{eqn:update1}, at time-step $\bar{t}(\omega)\in\mathbb{I}$, $\mu_{i,\bar{t}(\omega)}(\theta^{\star})$ for an agent $i\in\mathcal{V}$ satisfies:
\begin{equation}
\resizebox{0.85\hsize}{!}{$
\begin{aligned}
\mu_{i,\bar{t}(\omega)}(\theta^{\star})&\geq\frac{\eta(\omega)}{\sum\limits_{p=1}^{m}\min\{\{\mu_{j,\bar{t}(\omega)-1}(\theta_p)\}_{{j\in\mathcal{N}_i}},\pi_{i,\bar{t}(\omega)}(\theta_p)\}}\\
&\geq\frac{\eta(\omega)}{\sum\limits_{p=1}^{m}\pi_{i,\bar{t}(\omega)}(\theta_p)}=\eta(\omega),
\end{aligned}
$}
\end{equation}
where the last equality follows from the fact that the local belief vectors generated via \eqref{eqn:Bayes} are valid probability distributions over the hypothesis set $\Theta$ at each time-step, and hence $\sum\limits_{p=1}^{m}\pi_{i,\bar{t}(\omega)}(\theta_p)=1$. The above argument applies identically to each agent in $\mathcal{V}$. Furthermore, it is easily seen that based on \eqref{eqn:update2}, and a similar reasoning as above, identical conclusions can be drawn for each time-step $t>t'(\omega),t\in\mathbb{I}$ when the agents update their actual beliefs based on \eqref{eqn:update1}. This readily establishes \eqref{eqn:lowerbound}, and completes the proof. 
\end{proof}
\fi


\begin{figure}[t]
\begin{center}
%\hspace*{-1cm}
\begin{tikzpicture}
[->,shorten >=1pt,scale=.75,inner sep=1pt, minimum size=12pt, auto=center, node distance=3cm,
  thick, node/.style={circle, draw=black, thick},]
\tikzstyle{block1} = [rectangle, draw, fill=red!10, 
    text width=8em, text centered, rounded corners, minimum height=0.8cm, minimum width=1cm];
\node [circle, draw,fill=gray!30](n1) at (0,0)     (1)  {$1$};
\node [circle, draw](n2) at (2,0)     (2)  {$2$};
\node [circle, draw](n3) at (4,0)     (3)  {$3$};
\node [circle, draw](n4) at (6,0)     (4)  {$4$};
\node [circle, draw, fill=gray!30](n5) at (5,1.5)     (5)  {$5$};
\node [circle, draw](n6) at (5,-1.5)     (6)  {$6$};
\node [circle, draw, fill=gray!30](n7) at (3,-1.5)     (7)  {$7$};
\node (rect) at (2,0) () [draw=red, dashed, minimum width=3.6cm, minimum height=0.8cm] {};
\node (rect) at (4,-1.5) () [draw=blue, dashed, minimum width=2.2cm, minimum height=0.8cm] {};
\node (rect) at (6,0) () [draw=blue, dashed, minimum width=0.8cm, minimum height=0.8cm] {};
\node (rect) at (5,1.5) () [draw=ForestGreen, dashed, minimum width=0.8 cm, minimum height=0.8cm] {};
\draw [-, thick] (1) to (2);
\draw [-, thick] (2) to (3);
\draw [-, thick] (3) to (4);
\draw [-, thick] (7) to (6);
\draw [-,thick] (5) to [bend left=20] (4);
\draw [-,thick] (6) to [bend right=20] (4);
\end{tikzpicture}
\end{center}
\caption{The figure represents the network for the simulation example in Section \ref{sec:sim}. Based on the parameters of the model, Theorem \ref{thm:main} implies that the asymptotic rates of rejection of $\theta_2$ for the agents enclosed in the red, blue and green rectangles are dictated by the relative entropies of agents 1, 7 and 5, respectively, illustrating the agent-specific learning rate phenomenon.}
\label{fig:example}
\end{figure}
\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
%\includegraphics[scale=0.235]{ag3.jpg}&\includegraphics[scale=0.235]{ag4.jpg}\\
\end{tabular}
\end{center}
\caption{The figure plots the instantaneous rates of decay of the beliefs of agents $3$ and $4$ on the false hypothesis $\theta_2$ (given by $-\log{\mu_{i,t}(\theta_2)}/{t}, i\in\{3,4\}$), for the model described in Section \ref{sec:sim}. The parameter $\beta_{i,j}=a^{(d(i,j)+1)}$ in the above plots represents the factor by which the signal strength of agent $i$ is attenuated at the location of agent $j$.}   
\label{fig:plots}
\end{figure}
